DANCE: Differentiable Accelerator/Network Co-Exploration

To cope with the ever-increasing computational demand of the DNN execution, recent neural architecture search (NAS) algorithms consider hardware cost metrics into account, such as GPU latency. To further pursue a fast, efficient execution, DNN-specialized hardware accelerators are being designed for multiple purposes, which far-exceeds the efficiency of the GPUs. However, those hardware-related metrics have been proven to exhibit non-linear relationships with the network architectures. Therefore it became a chicken-and-egg problem to optimize the network against the accelerator, or to optimize the accelerator against the network. In such circumstances, this work presents DANCE, a differentiable approach towards the co-exploration of the hardware accelerator and network architecture design. At the heart of DANCE is a differentiable evaluator network. By modeling the hardware evaluation software with a neural network, the relation between the accelerator architecture and the hardware metrics becomes differentiable, allowing the search to be performed with backpropagation. Compared to the naive existing approaches, our method performs co-exploration in a significantly shorter time, while achieving superior accuracy and hardware cost metrics.

==> cifar.tex <==
\begin{table*}[]
    \centering
    %\small
    \begin{tabular}{c|c|c|c|l|c|c|c|c|c}
    \multirow{2}{*}{$HW\_{Cost}$} & \multicolumn{3}{c|}{Cost Hyperparam.} & \multirow{2}{*}{~~~~~~~~~~~~~~~~~~~~~~~Method} &\multirow{2}{*}{ Acc.} & \multirow{2}{*}{Latency} & \multirow{2}{*}{Energy} & \multirow{2}{*}{EADP} \\
    &$\lambda_L$&$\lambda_E$&$\lambda_A$&& \\
    \hline
      \multirow{4}{*}{$Cost_{HW\_EDAP}$} &  \multicolumn{3}{c|}{\multirow{4}{*}{N/A}}  & Baseline (No penalty) + HW$^*$ & 94.5\% & 5ms & 13.5mJ & 133 \\ 
      & \multicolumn{3}{c|}{} &   Baseline (Flops penalty) + HW &  94.2\% & 3.08ms &  11.8mJ  & 94.8 \\
      & \multicolumn{3}{c|}{} &  \nasname (w/o FF$^*$) & 93.1\%  &  \\
      & \multicolumn{3}{c|}{}&  \nasname (w/ FF) & 94.4\%  & 2.77ms & 10.2mJ &  74.0 \\
      \hline
      
      \multirow{4}{*}{\makecell {$Cost_{HW\_linear}$ \\ (Balanced)}} & \multirow{4}{*}{4.1} &\multirow{4}{*}{4.8} &\multirow{4}{*}{1.0} & Baseline (No penalty) + HW &&&\\ 
      & && &   Baseline (Flops penalty) + HW &  &  & \\
      & && &  \nasname (w/o FF) &  && &  \\      
      & && &  \nasname (w/ FF) & 94.26\%  & 2.17ms & 7.82mJ & 44.4 \\
      \hline
      
      \multirow{4}{*}{\makecell {$Cost_{HW\_linear}$ \\ (Latency-Oriented)} } & \multirow{4}{*}{4.9} &\multirow{4}{*}{3.9} &\multirow{4}{*}{1.0}& Baseline (No penalty) + HW &&&\\ 
      & && &   Baseline (Flops penalty) + HW &  &  &  \\
      & && &  \nasname (w/o FF) &  && &  \\
      & && &  \nasname (w/ FF) & 93.4\% & 1.02ms & 3.99mJ & 3.42mm$^2$ \\
      \hline
      
      \multirow{4}{*}{\makecell {$Cost_{HW\_linear}$ \\ (Energy-Oriented)} } &   \multirow{4}{*}{0.7} &\multirow{4}{*}{8.4} &\multirow{4}{*}{1.0}  & Baseline (No penalty) + HW &&&\\ 
      & && &   Baseline (Flops penalty) + HW &  &  & \\
      & && &  \nasname (w/o FF) &  && &  \\
            & && &  \nasname (w/ FF) & 93.4\% & 1.33ms & 5.10mJ & 3.42mm$^2$  \\
              \hline 
        \multicolumn{9}{r}{\tiny*HW: Hardware accelerator, designed using the hardware generation tool after the NAS.} \\
        \multicolumn{9}{r}{\tiny*FF: Feature Forwarding.} \\
    \end{tabular}
    \caption{Performance of DANCE on CIFAR-10}
    \label{tbl:cifar}
\end{table*}



\begin{table*}[]
    \centering
    %\small
    \begin{tabular}{c|p{6mm}|p{6mm}|p{6mm}|l|c|c|c|c|c}
    \multirow{2}{*}{$HW\_{Cost}$} & \multicolumn{3}{c|}{Cost Hyperparam.} & \multirow{2}{*}{~~~~~~~~~~~~~~~~~~~~~~~Method} & Acc. & Latency & Energy & \multirow{2}{*}{EDAP} \\
    &$\lambda_L$&$\lambda_E$&$\lambda_A$&&  (\%) & (ms) & (mJ) & \\
    \hline
      \multirow{2}{*}{$Cost_{HW\_EDAP}$} &  \multicolumn{3}{c|}{\multirow{2}{*}{N/A}}  & Baseline (No penalty) + HW$^*$ & 94.5\% & 5ms & 13.5mJ & 133 \\ 
      & \multicolumn{3}{c|}{} &   Baseline (Flops penalty) + HW &  94.2\% & 3.08ms &  11.8mJ  & 94.8 \\
      \hline
     
      \multirow{2}{*}{$Cost_{HW\_EDAP}$} & \multicolumn{3}{c|}{\multirow{2}{*}{N/A}} & 
      \nasname (w/o FF$^*$) & 93.1\%  &  \\
      & \multicolumn{3}{c|}{}&  \nasname (w/ FF) & 94.4\%  & 2.77ms & 10.2mJ &  74.0 \\
      \hline
      
      \multirow{2}{*}{\makecell {$Cost_{HW\_linear}$ \\ (Balanced)}} & \multirow{2}{*}{4.1} &\multirow{2}{*}{4.8} &\multirow{2}{*}{1.0} &
      \nasname (w/o FF) &  && &  \\      
      & && &  \nasname (w/ FF) & 94.26\%  & 2.17ms & 7.82mJ & 44.4 \\
      \hline
      
      \multirow{2}{*}{\makecell {$Cost_{HW\_linear}$ \\ (Latency-Oriented)} } & \multirow{2}{*}{4.9} &\multirow{2}{*}{3.9} &\multirow{2}{*}{1.0}&
      \nasname (w/o FF) &  && &  \\
      & && &  \nasname (w/ FF) & 94.29\% & 2.22ms & 7.96mJ & 46.2  \\
      \hline
      
      \multirow{2}{*}{\makecell {$Cost_{HW\_linear}$ \\ (Energy-Oriented)} } &   \multirow{2}{*}{0.7} &\multirow{2}{*}{8.4} &\multirow{2}{*}{1.0} & \nasname (w/o FF) &  && &  \\
            & && &  \nasname (w/ FF) & 93.43 & 1.43ms & 5.00 & 18.7  \\
              \hline 
        \multicolumn{9}{r}{\small*HW: Hardware accelerator, designed using the hardware generation tool after the NAS.} \\
        \multicolumn{9}{r}{\small*FF: Feature Forwarding.} \\
    \end{tabular}
    \caption{Performance of DANCE on CIFAR-10}
    \label{tbl:cifar}
\end{table*}}

==> trash.tex <==

\begin{comment}


\JL{this is too sudden. need more build-up for claiming importance of latency?, or energy}
To address the issue,\JS{accelrator has to be explained. tpu?} hardware-related metrics\JS{this term sucks} such as latency or energy efficiency are becoming major targets of optimizations. 
Often, this is achieved from building more efficient networks~\cite{efficientnet, mobilenet, mobilenetv2, proxylessNAS, @}, designing hardware accelerators~\cite{tpu, eyeriss, shidiannao, @}, and various optimizations~\cite{quantization, sparse, compression}.

\JS{explain the need for codesign. current: separate design}
Designing hardware accelerators for DNNs, or neural processing units (NPU) is a popular approach taken to cope with the exploding computation requirements. 
As modern CPUs, or even GPUs turned out to be inefficient for executing DNNs, a number of architectures have been proposed to optimize the latency as well as the energy consumption.
Oriented towards the accelerating matrix multiplication as the core operation, they improve various features such as data reuse~\cite{eyeriss}, exploiting sparsity~\cite{scnn}, or quantizations~\cite{bitfusion, olaccel}.
\JS{use easier HW techniques}

\end{comment}





with separated HW generation and metric evaluation network. 
At the top is a module that generates the network and trains it at the same time, as in many other differentiable neural architecture search methods~\cite{darts, proxylessnas, fbnas}.
While generating/training the network, the network architecture is passed to the accelerator generator, which performs design-space exploration\JL{the term is not familiar to AI world} and searches for the optimal accelerator design. 
Than the evaluation network evaluates the accelerator design along with the network. 
The HW metrics are output from the evaluation network, and used for the loss function.
Note that both modules are modeled as neural networks, and thus fully differentiable.
An example loss function is displayed below:
\begin{equation}
    L_{sep} = L_{CE} + \lambda L_{HW}(Eval(\alpha, HWgen(\alpha)))
\end{equation}
Where $L_{CE}$ is the cross-entropy loss assuming the network under search is for a classification problem. 
$Eval()$ and $HWgen()$ are evaluation and HW accelerator generator network\JS{gumble softmax for HWgen()}, respectively. 
Lastly, $L_{HW}$ is a HW metric loss function that defines the HW metrics of interest. 
For example, EDAP (product of energy, delay, and area) output from the evaluation network can be used. \JL{EDAP is too difficult}
Refer to Section~\ref{sec:eval} for the HW metric loss functions we have tested.


\figurename~\ref{fig:nas-unified} shows another version of \nasname, with unified accelerator generation and metric evaluation network. 
In this version, the unified accelerator generator outputs both the accelerator design and the HW metrics.
Therefore the loss now becomes
\begin{equation}
    L_{unified} = L_{CE} + \lambda L_{HW}(\alpha, HWgen(\alpha))
\end{equation}
The unified model does not undergo transition of information between the two approximated neural network, and can be better modeled. 
However, an evaluation network is still needed to ensure that the accelerator design and the HW metric have the correct correlation.\JL{why unified?}

\JL{explain $L_{HW}$ as EDAP, linear comb, etc}
Depending on the computation, it can be a user-defined function such as EDAP (Energy-Delay-Area product), or linear combination of the ...

\subsection{Metric Evaluation Network}
\label{eval_net}
Evaluation network estimates the HW metrics.
Effectively, the network functions as a linear approximations for the neural architecture to the HW accelerators so that the neural architecture can be updated using gradient-based optimizers.

Since the HW accelerator cannot be actually implemented every time a configuration is generated, approximate methods such as \JS{what the simulator?}simulators~\cite{scalesim}, or analyzer~\cite{maestro, timeloop} can be used.
In this work, we utilize a state-of-the-art analyzer Timeloop~\cite{timeloop}.
Originally designed as a design-space optimizing tool, it accepts layer configurations and HW configurations as inputs, and outputs latency, area, and energy consumptions. 
Using design a separate network for each of the three metrics. 
Even though we can employ a multi-headed architecture to reduce the overall model size, the size of the metric evaluation network is dwarfed by the backbone NAS network, and is not add significant computational overhead to the overall system.
For all networks, we define the loss function $L$ as below.
\begin{equation}
    L = (1 - \frac{\hat{y}}{y})^2
\end{equation}
\JS{toy example?}\JL{is there a name for the loss function?}
Where $\hat{y}$ is the output of the metric evaluation network, and $y$ is the ground-truth metric generted by Timeloop. 
While we could use typical loss functions such as MSE, it has a problem of falsely heavy-weighing the highly values metrics. \JL{err plot?}
For example, the latency values outputted within our search space ranges from @@@10K~1M cycles (at 1ns per cycle).
If we use MSE, we are regarding the 1K cycle error out of 10K and 1M cycles as the same, which would give unfair favor towards modeling the long-cycle situations more correct. 

We model the metric evaluation network as a MLP (Multi-Layer Perceptron) as shown in \figurename~\ref{fig:evalnet}.
We use five hidden layers, where each layer is followed by ReLU and batch normalization. 
Also, even though the network itself has a small number of layers, we add residual connections~\cite{resnet} because the network will be act as if it is the last few layers of the network under search.



\subsection{Accelerator Generation Network}
%We also use Timeloop DSE tool~\cite{timeloop} for accelerator generation. 
%It does exhaustive search while performing branch-and-bound to prune the search space, but takes ~20 minutes per search~\cite{timeloop}.
We choose \JS{eyeriss?, PE?, register? need it in background} eyeriss-like architecture as the backbone HW acclerator, and the PE array width, PE array height, and register file size are used as tunable HW parameters. 
We use similar MLP network as in the metric evaluation network with residual connections.
To change DSE into an optimization problem, we forward the output to the evaluation network, and let the network optimize the HW metric of interest. 

The baseline Timeloop~\cite{timeloop} performs exhaustive search and applies branch-and-bound techniques to prune the search space. 
However, it is reported that the search needs too many evaluation runs, and requires a few minutes per search.
However, the network-approximated generation finishes in a sub-second scale, providing a low enough latency to be used in an architecture search. 



\begin{comment}


It is formulated as a multi-task network, where one task outputs the hardware design (loop order, number of processing elements, register file size) and the other task outputs the cost metrics (latency, chip area, energy consumption).
The unified evaluator network is composed of @ linear layers with slightly more hidden layer depth than the hardware generation network or the analysis network considering the increased problem complexity. 
While the unified evaluator network solves the discrete intermediate value problem, it introduces another hyperparameter. 
The loss for traning the unified evaluator is as follows:
\begin{equation}
\mathcal{L}oss_{uni} = \mathcal{L}oss_{CE\_HW} + \lambda_{uni}\mathcal{L}oss_{eval}
\end{equation}
$\lambda_{uni}$ sets the balance between the hardware generation and the cost analysis where we use an empirical value of @@.

\end{comment}


\begin{comment}

\subsection{One-Step Evaluator Network}
Our second design, One-step evaluator merges the path of the cost metric from two-steps into a single step.
This solves the discrete value problem from the previous section, at the cost of making the problem slightly more complicated.

\figurename~\ref{fig:unified} shows the architecture of the One-step evaluator network. 
The hardware generation network remains, but the analysis network takes only the architecture parameters instead of the concatenated value.
It is trained to output the cost metrics for the optimal accelerator design given the network parameters, without outputting the actual accelerator design. 
We name this the optimal accelerator analysis network.
While we could have designed the one-step evaluator as a multi-task network, the complexity of the networks were already small enough and decided that return from the effort would not be significant.
The network is a five-layer regression with width of 256 and residual connections.
It has been trained for 500 Epochs with batch size 128 using Adam optimizer, there the learning rate starts at 0.0001 and decreases by $0.1\times$ at 50th and 100th epoch.


\end{comment}

